Massively Multilingual Transfer for NER

In cross-lingual transfer, NLP models over one or more source languages are applied to a low-resource target language. While most prior work has used a single source model or a few carefully selected models, here we consider a `massive' setting with many such models. This setting raises the problem of poor transfer, particularly from distant languages. We propose two techniques for modulating the transfer, suitable for zero-shot or few-shot learning, respectively. Evaluating on named entity recognition, we show that our techniques are much more effective than strong baselines, including standard ensembling, and our unsupervised method rivals oracle selection of the single best individual model.

==> figs/topk.tex <==
\begin{figure}[t]
	\centering
	\begin{tikzpicture}[scale=0.8]
	\begin{axis}[
	%axis x line=center,
	legend pos=south east,
	xtick pos=left,
	ytick pos=left,
	grid=both,
	grid style={dashed,gray!30},
	axis y line*=left,
	axis x line*=left,
	ylabel near ticks,
	xlabel near ticks,
	xlabel=\#source languages,
	ylabel=mean \fone over $41$ langs.,
	%axis y line=none,
	%hide y axis,
	xmin=-100,xmax=450,
	ymin=55, ymax=85,
	xtick={0, 100, 200, 300, 400},
	ytick={60,65,70,75,80},
	xticklabels={1, 2, 5, 10, 40},
	%xticklabel style={rotate=20},
	]
	
	\addplot[
	scatter/classes={a={blue}, b={red,mark=square*}},
	scatter,
	only marks,
	%grid=both,
	visualization depends on=\thisrow{ey} \as \myshift,
	every node near coord/.append style = {shift={(axis direction
			cs:0,\myshift)}},
	scatter src=explicit symbolic,
	%nodes near coords*={\Label},
	visualization depends on={value \thisrow{label} \as \Label},
	]%
	plot [error bars/.cd, y dir = both, y explicit]
	table[meta=class, x=x, y=y, y error=ey]{
		x   y	ey  class	label
		-15	74.8	7.3	a	top$1$
		15	64.2	7.7	b	unif$1$
		85	76.8	7.5	a	top$2$
		115	69.1	7.6	b	unif$2$
		185	77.8	6.1	a	top$5$
		215	73.3	7.5	b	unif$5$
		285	77.9	6.3	a	top$10$
		315	74.3	7.2	b	unif$10$
		385	77.4	6.3	a	top$40$
		415	76.0	6.4	b	unif$40$
	};
	\legend{\fone selection, random selection}
	\end{axis}
	\end{tikzpicture}
	\caption{The mean and standard deviation \fone performance of \ssagg over the $41$ languages categorised by the number of source languages used for transfer. The top $k$ languages are chosen either based on \fone performance of the source model on the target language (\mycircle{blue}), or randomly (\mysquare{red}).}
	\label{fig:topk}
\end{figure}

==> figs/unk.tex <==
\begin{table*}
	\footnotesize
	\centering
	%\resizebox{\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{llllllllllllllllllllllllllllllllllllllllll}
lang &af &ar &bg &bn &bs &ca &cs &da &de &el &en &es &et &fa &fi &fr &he &hi &hr &hu &id &it &lt &lv &mk &ms &nl &no &pl &pt &ro &ru &sk &sl &sq &sv &ta &tl &tr &uk &vi\\
unkpersent &1.25 &0.47 &0.89 &0.4 &1.11 &1.05 &1.41 &0.87 &1.07 &1.21 &1.22 &0.72 &1.03 &0.25 &1.16 &1.08 &0.73 &0.64 &1.05 &1.25 &0.74 &1.29 &0.95 &1.29 &0.76 &0.78 &0.88 &0.94 &0.98 &0.88 &0.95 &0.83 &1.15 &1.15 &1.56 &0.69 &0.96 &0.6 &1.52 &1.1 &0.81\\
unkinner &28 &22 &14 &49 &19 &17 &12 &25 &18 &07 &19 &18 &19 &28 &21 &27 &31 &14 &18 &24 &28 &13 &21 &21 &12 &28 &19 &21 &17 &17 &27 &24 &17 &16 &07 &23 &28 &4 &28 &24 &17\\
unkinnonner &11 &14 &14 &28 &16 &31 &22 &11 &13 &18 &24 &22 &16 &1 &16 &24 &09 &22 &15 &15 &19 &23 &16 &23 &9 &23 &13 &12 &15 &27 &23 &16 &19 &21 &28 &08 &16 &36 &24 &17 &28
\end{tabular}
%}
\end{table*}

==> nerdatasets.tex <==
\begin{table}
\begin{tabular}{l|p{3cm}l}
\textbf{\#train} & \quad\quad \textbf{(\#dev, \#test)}  & \\
\hline
  & \textbf{10k} & \textbf{1k} \\
\hline
\textbf{5k} & - & \lang{af}, \lang{hi}, \lang{sq}\\
\hline
\textbf{10k} & \lang{lt}, \lang{lv}, \lang{et}, \lang{sl} & \lang{mk}, \lang{tl}\\
\hline
\textbf{15k} & \lang{et}, \lang{sl} & \lang{bs}, \lang{ta} \\
\hline
\textbf{20k} & \parbox{3cm}{\lang{ar}, \lang{bg}, \lang{ca}, \lang{cs}, \lang{da}, \lang{de}, \lang{el}, \lang{en}, \lang{es}, \lang{fa}, \lang{fi}, \lang{fr}, 
\lang{he}, \lang{hr}, \lang{hu}, \lang{id}, \lang{it}, \lang{nl}, \lang{no}, \lang{pl}, \lang{pt}, \lang{ro}, \lang{ru}, \lang{sk}, \lang{sv}, \lang{tr}, \lang{uk}, \lang{vi}}& \lang{ms}\\
\end{tabular}
\caption{The training and dev/test size of the NER datasets in terms of the number of sentences. The datasets are compiled from the original datasets (Pan e. al, 2017)
for our experiments. To see the dataset sizes in low-resource and high-resource settings see \tabref{tab:datasetssetting}.}
\label{tab:datasets}
\end{table}

==> top5.tex <==
\begin{table*}
\begin{tabular}{l|l}
	  &  top $5$ langs. \\
\hline
\lang{af} &  \lang{pl}, \lang{nl}, \lang{no}, \lang{id}, \lang{hu} \\
\lang{ar} &  \lang{de}, \lang{fa}, \lang{mk}, \lang{nl}, \lang{hi} \\
\lang{bg} &  \lang{ru}, \lang{uk}, \lang{mk}, \lang{ar}, \lang{ta} \\
\lang{bn} &  \lang{ta}, \lang{tl}, \lang{hi}, \lang{ar}, \lang{ms} \\
\lang{bs} &  \lang{hr}, \lang{sk}, \lang{pl}, \lang{cs}, \lang{nl} \\
\lang{ca} &  \lang{es}, \lang{pt}, \lang{fr}, \lang{it}, \lang{en} \\
\lang{cs} &  \lang{sk}, \lang{pl}, \lang{no}, \lang{hr}, \lang{it} \\
\lang{da} &  \lang{fi}, \lang{no}, \lang{nl}, \lang{sk}, \lang{it} \\
\lang{de} &  \lang{da}, \lang{no}, \lang{fr}, \lang{hr}, \lang{hu} \\
\lang{el} &  \lang{ar}, \lang{fr}, \lang{fa}, \lang{sk}, \lang{de} \\
\lang{en} &  \lang{pt}, \lang{tr}, \lang{fr}, \lang{pl}, \lang{ro} \\
\end{tabular}
\begin{tabular}{l|l}
	  &  top $5$ langs. \\
\hline
\lang{es} &  \lang{nl}, \lang{pt}, \lang{fr}, \lang{pl}, \lang{hr} \\
\lang{et} &  \lang{fi}, \lang{hu}, \lang{da}, \lang{no}, \lang{cs} \\
\lang{fa} &  \lang{nl}, \lang{de}, \lang{no}, \lang{es}, \lang{hi} \\
\lang{fi} &  \lang{pl}, \lang{da}, \lang{hu}, \lang{et}, \lang{hr} \\
\lang{fr} &  \lang{nl}, \lang{it}, \lang{es}, \lang{pt}, \lang{no} \\
\lang{he} &  \lang{el}, \lang{fr}, \lang{hr}, \lang{es}, \lang{mk} \\
\lang{hi} &  \lang{bn}, \lang{ar}, \lang{fa}, \lang{id}, \lang{he} \\
\lang{hr} &  \lang{sl}, \lang{bs}, \lang{es}, \lang{hu}, \lang{pl} \\
\lang{hu} &  \lang{et}, \lang{fi}, \lang{no}, \lang{tr}, \lang{fr} \\
\lang{id} &  \lang{it}, \lang{fr}, \lang{ms}, \lang{nl}, \lang{cs} \\
\lang{it} &  \lang{fr}, \lang{pl}, \lang{da}, \lang{en}, \lang{nl} \\
\end{tabular}
\begin{tabular}{l|l}
	  &  top $5$ langs. \\
\hline
\lang{lt} &  \lang{nl}, \lang{pl}, \lang{no}, \lang{fi}, \lang{hr} \\
\lang{lv} &  \lang{nl}, \lang{es}, \lang{lt}, \lang{sk}, \lang{pt} \\
\lang{mk} &  \lang{uk}, \lang{bg}, \lang{ru}, \lang{no}, \lang{de} \\
\lang{ms} &  \lang{pl}, \lang{nl}, \lang{fr}, \lang{id}, \lang{ca} \\
\lang{nl} &  \lang{da}, \lang{it}, \lang{pl}, \lang{bs}, \lang{de} \\
\lang{no} &  \lang{fi}, \lang{nl}, \lang{pl}, \lang{fr}, \lang{hr} \\
\lang{pl} &  \lang{it}, \lang{no}, \lang{nl}, \lang{tr}, \lang{cs} \\
\lang{pt} &  \lang{fr}, \lang{es}, \lang{pl}, \lang{no}, \lang{it} \\
\lang{ro} &  \lang{pt}, \lang{es}, \lang{fr}, \lang{nl}, \lang{en} \\
\lang{ru} &  \lang{uk}, \lang{bg}, \lang{mk}, \lang{es}, \lang{pt} \\
\lang{sk} &  \lang{pl}, \lang{ca}, \lang{cs}, \lang{es}, \lang{pt} \\
\end{tabular}
\begin{tabular}{l|l}
	  &  top $5$ langs. \\
\hline
\lang{sl} &  \lang{hr}, \lang{cs}, \lang{it}, \lang{pl}, \lang{sk} \\
\lang{sq} &  \lang{it}, \lang{nl}, \lang{pl}, \lang{ro}, \lang{no} \\
\lang{sv} &  \lang{fi}, \lang{no}, \lang{da}, \lang{sk}, \lang{de} \\
\lang{ta} &  \lang{he}, \lang{ru}, \lang{ar}, \lang{tr}, \lang{fi} \\
\lang{tl} &  \lang{en}, \lang{ca}, \lang{vi}, \lang{ro}, \lang{nl} \\
\lang{tr} &  \lang{no}, \lang{fi}, \lang{pl}, \lang{et}, \lang{nl} \\
\lang{uk} &  \lang{ru}, \lang{mk}, \lang{bg}, \lang{no}, \lang{es} \\
\lang{vi} &  \lang{ro}, \lang{en}, \lang{es}, \lang{ca}, \lang{pt} \\
\\
\\
\\
\end{tabular}
\caption{Top 5 performing models trained on a language in a high-resource setting, tested on the training set of other languages in low-resource setting (100 sentences).
For example models trained on \lang{ro}, \lang{en}, \lang{es}, \lang{ca} and \lang{pt} performed best in terms of F1 score on 100 training sentences of \lang{vi}.}
\label{tab:top5langs}
\end{table*}
